Improvements to deep convolutional neural networks for LVCSR

Deep Convolutional Neural Networks (CNNs) are more powerful than Deep Neural Networks (DNN), as they are able to better reduce spectral variation in the input signal. This has also been confirmed experimentally, with CNNs showing improvements in word error rate (WER) between 4-12% relative compared to DNNs across a variety of LVCSR tasks. In this paper, we describe different methods to further improve CNN performance. First, we conduct a deep analysis comparing limited weight sharing and full weight sharing with state-of-the-art features. Second, we apply various pooling strategies that have shown improvements in computer vision to an LVCSR speech task. Third, we introduce a method to effectively incorporate speaker adaptation, namely fMLLR, into log-mel features. Fourth, we introduce an effective strategy to use dropout during Hessian-free sequence training. We find that with these improvements, particularly with fMLLR and dropout, we are able to achieve an additional 2-3% relative improvement in WER on a 50-hour Broadcast News task over our previous best CNN baseline. On a larger 400-hour BN task, we find an additional 4-5% relative improvement over our previous best CNN baseline.

==> experiments.tex <==
\section{Experiments \label{sec:experiments}}

Experiments are conducted on a 50-hour English Broadcast News task \cite{bedk:nn}. The acoustic models are trained on 50 hours of data from the 1996 and 1997 English Broadcast News Speech Corpora. Results are reported on the EARS \texttt{dev04f} set. 

The baseline CNN system is trained with 40 dimensional log mel-filterbank coefficients, which are global mean-and -variance normalized. The architecture of the CNN is similar to \cite{tsainath:cnnLVCSR}, which was found to be optimal for broadcast news. Specifically, the CNN has 2 fully connected layers with 256 output targets, and 3 fully connected layers with 1,024 hidden units per layer. The final softmax-layer consists of 512 output targets. 

Following a recipe similar to \cite{tsainath:dbnHybrid}, during fine-tuning, after one pass through the data, loss is measured on a held-out set and the learning rate is reduced by a factor of 2 if the held-out loss has not improved sufficiently over the previous iteration. Training stops after we have reduced the step size 5 times. All DNNs and CNNs are trained with cross-entropy, and results are reported in a hybrid setup.

